From Qubits to Rhythm: Exploring Quantum Random Walks in Rhythmspaces

A quantum computing algorithm for rhythm generation is presented, which aims to expand and explore quantum computing applications in the arts, particularly in music. The algorithm maps quantum random walk trajectories onto a rhythmspace -- a 2D interface that interpolates rhythmic patterns. The methodology consists of three stages. The first stage involves designing quantum computing algorithms and establishing a mapping between the qubit space and the rhythmspace. To minimize circuit depth, a decomposition of a 2D quantum random walk into two 1D quantum random walks is applied. The second stage focuses on biasing the directionality of quantum random walks by introducing classical potential fields, adjusting the probability distribution of the wave function based on the position gradient within these fields. Four potential fields are implemented: a null potential, a linear field, a Gaussian potential, and a Gaussian potential under inertial dynamics. The third stage addresses the sonification of these paths by generating MIDI drum pattern messages and transmitting them to a Digital Audio Workstation (DAW). This work builds upon existing literature that applies quantum computing to simpler qubit spaces with a few positions, extending the formalism to a 2D x-y plane. It serves as a proof of concept for scalable quantum computing-based generative random walk algorithms in music and audio applications. Furthermore, the approach is applicable to generic multidimensional sound spaces, as the algorithms are not strictly constrained to rhythm generation and can be adapted to different musical structures.

==> Definitions/journalnames.tex <==
% Updated 18 December 2024 used for Y2025
%% --------------------------------------------------------------------
%\DeclareOption{}{%%
%		\gdef\@journal{}
%		\gdef\@journalfull{}
%		\gdef\@journalshort{}
%		\gdef\@doiabbr{}
%		\gdef\@ISSN{}
%		\gdef\@continuouspages{yes}
%		\gdef\@societyowner{}
%}
%% --------------------------------------------------------------------
%% Fields meanings:
%% - Option name: Journal website name (used in URL)
%% - @journal: Journal website name (used in URL)
%% - @journalshort: Short Name (ISO4)
%% - @journalfull: Journal full name
%% - @doiabbr: DOI abbreviation of the journal used in DOI numbers 10.32604/journalnameXXXX
%% - @ISSN: Journal E-ISSN number
%% - @continuouspages: use 	\gdef\@continuouspages{yes} for journals that use pagination
%% - @societyowner: Name of society owning the journal (for society journals)
%% --------------------------------------------------------------------
\DeclareOption{biocell}{%
	\gdef\@journal{biocell}
	\gdef\@journalshort{Biocell}
	\gdef\@journalfull{Biocell}
	\gdef\@doiabbr{biocell}
	\gdef\@ISSN{1667-5746}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{chd}{%
	\gdef\@journal{chd}
	\gdef\@journalshort{Congenit Heart Dis}
	\gdef\@journalfull{Congenital Heart Disease}
	\gdef\@doiabbr{chd}
	\gdef\@ISSN{1747-0803}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cmc}{%
 	\gdef\@journal{cmc}
	\gdef\@journalshort{Comput Mater Contin.}
	\gdef\@journalfull{Computers, Materials \& Continua}
	\gdef\@doiabbr{cmc}	\gdef\@ISSN{1546-2226}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cmes}{%
 	\gdef\@journal{cmes}
	\gdef\@journalshort{Comput Model Eng Sci}
	\gdef\@journalfull{Computer Modeling in Engineering \& Sciences}
	\gdef\@doiabbr{cmes}
	\gdef\@ISSN{1526-1506}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{csse}{%
 	\gdef\@journal{csse}
	\gdef\@journalshort{Comput Syst Sci Eng}
	\gdef\@journalfull{Computer Systems Science and Engineering}
	\gdef\@doiabbr{csse}
	\gdef\@ISSN{0267-6192}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% ISSN (print)
\DeclareOption{dedt}{%
 	\gdef\@journal{dedt}
	\gdef\@journalshort{Digit Eng Digit Twin}
	\gdef\@journalfull{Digital Engineering and Digital Twin}
	\gdef\@doiabbr{dedt}
	\gdef\@ISSN{ }
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% No ISSN
\DeclareOption{ee}{%
 	\gdef\@journal{ee}
	\gdef\@journalshort{Energy Eng}
	\gdef\@journalfull{Energy Engineering}
	\gdef\@doiabbr{ee}
	\gdef\@ISSN{1546-0118}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{fdmp}{%
 	\gdef\@journal{fdmp}
	\gdef\@journalshort{Fluid Dyn Mater Process}
	\gdef\@journalfull{Fluid Dynamics \& Materials Processing}
	\gdef\@doiabbr{fdmp}
	\gdef\@ISSN{1555-2578}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{fhmt}{%
 	\gdef\@journal{fhmt}
	\gdef\@journalshort{Front Heat Mass Transf}
	\gdef\@journalfull{Frontiers in Heat and Mass Transfer}
	\gdef\@doiabbr{fhmt}
	\gdef\@ISSN{2125-8629}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% ISSN (print)
\DeclareOption{iasc}{%
 	\gdef\@journal{iasc}
	\gdef\@journalshort{Intell Autom Soft Comput}
	\gdef\@journalfull{Intelligent Automation \& Soft Computing}
	\gdef\@doiabbr{iasc}
	\gdef\@ISSN{2326-005X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{icces}{%
 	\gdef\@journal{icces}
	\gdef\@journalshort{Int Conf Comput Exp Eng Sci}
	\gdef\@journalfull{The International Conference on Computational \& Experimental Engineering and Sciences}
	\gdef\@doiabbr{icces}
	\gdef\@ISSN{1993-2815}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ijmhp}{%
 	\gdef\@journal{ijmhp}
	\gdef\@journalshort{Int J Ment Health Promot}
	\gdef\@journalfull{International Journal of Mental Health Promotion}
	\gdef\@doiabbr{ijmhp}
	\gdef\@ISSN{2049-8543}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jai}{%
 	\gdef\@journal{jai}
	\gdef\@journalshort{J Artif Intell}
	\gdef\@journalfull{Journal on Artificial Intelligence}
	\gdef\@doiabbr{jai}
	\gdef\@ISSN{2579-003X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jbd}{%
 	\gdef\@journal{jbd}
	\gdef\@journalshort{J Big Data}
	\gdef\@journalfull{Journal on Big Data}
	\gdef\@doiabbr{jbd}
	\gdef\@ISSN{2579-0056}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jbic}{%
 	\gdef\@journal{jbic}
	\gdef\@journalshort{J Blockchain Intell Comput}
	\gdef\@journalfull{Journal of Blockchain and Intelligent Computing}
	\gdef\@doiabbr{jbic}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% No ISSN
\DeclareOption{jcs}{%
 	\gdef\@journal{jcs}
	\gdef\@journalshort{J Cyber Secur}
	\gdef\@journalfull{Journal of Cyber Security}
	\gdef\@doiabbr{jcs}
	\gdef\@ISSN{2579-0064}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jihpp}{%
 	\gdef\@journal{jihpp}
	\gdef\@journalshort{J Inf Hiding Priv Prot}
	\gdef\@journalfull{Journal of Information Hiding and Privacy Protection}
	\gdef\@doiabbr{jihpp}
	\gdef\@ISSN{2637-4226}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jimh}{%
 	\gdef\@journal{jimh}
	\gdef\@journalshort{JIMH}
	\gdef\@journalfull{Journal of Intelligent Medicine and Healthcare}
	\gdef\@doiabbr{jimh}
	\gdef\@ISSN{2837-634X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jiot}{%
 	\gdef\@journal{jiot}
	\gdef\@journalshort{J Internet Things}
	\gdef\@journalfull{Journal on Internet of Things}
	\gdef\@doiabbr{jiot}
	\gdef\@ISSN{2579-0080}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jnm}{%
 	\gdef\@journal{jnm}
	\gdef\@journalshort{J New Media}
	\gdef\@journalfull{Journal of New Media}
	\gdef\@doiabbr{jnm}
	\gdef\@ISSN{2579-0129}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jpm}{%
 	\gdef\@journal{jpm}
	\gdef\@journalshort{J Polym Mater}
	\gdef\@journalfull{Journal of Polymer Materials}
	\gdef\@doiabbr{jpm}
	\gdef\@ISSN{0976-3449}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jqc}{%
 	\gdef\@journal{jqc}
	\gdef\@journalshort{J Quantum Comput}
	\gdef\@journalfull{Journal of Quantum Computing}
	\gdef\@doiabbr{jqc}
	\gdef\@ISSN{2579-0145}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jrm}{%
 	\gdef\@journal{jrm}
	\gdef\@journalshort{J Renew Mater}
	\gdef\@journalfull{Journal of Renewable Materials}
	\gdef\@doiabbr{jrm}
	\gdef\@ISSN{2164-6341}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{or}{%
 	\gdef\@journal{or}
	\gdef\@journalshort{Oncol Res}
	\gdef\@journalfull{Oncology Research}
	\gdef\@doiabbr{or}
	\gdef\@ISSN{1555-3906}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{phyton}{%
 	\gdef\@journal{phyton}
	\gdef\@journalshort{Phyton-Int J Exp Bot}
	\gdef\@journalfull{Phyton-International Journal of Experimental Botany}
	\gdef\@doiabbr{phyton}
	\gdef\@ISSN{1851-5657}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{po}{%
 	\gdef\@journal{po}
	\gdef\@journalshort{Psycho-Oncologie}
	\gdef\@journalfull{Psycho-Oncologie}
	\gdef\@doiabbr{po}
	\gdef\@ISSN{1778-381X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{rig}{%
 	\gdef\@journal{rig}
	\gdef\@journalshort{Rev Int Géomatique}
	\gdef\@journalfull{Revue Internationale de Géomatique}
	\gdef\@doiabbr{rig}
	\gdef\@ISSN{2116-7060}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sdhm}{%
 	\gdef\@journal{sdhm}
	\gdef\@journalshort{Struct Durab Health Monit}
	\gdef\@journalfull{Structural Durability \& Health Monitoring}
	\gdef\@doiabbr{sdhm}
	\gdef\@ISSN{1930-2991}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sv}{%
 	\gdef\@journal{sv}
	\gdef\@journalshort{Sound Vib}
	\gdef\@journalfull{Sound \& Vibration}
	\gdef\@doiabbr{sv}
	\gdef\@ISSN{2693-1443}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{notspecified}{%
	\gdef\@journal{notspecified}
	\gdef\@journalfull{Journal Not Specified}
	\gdef\@journalshort{Journal Not Specified}
	\gdef\@doiabbr{journal}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{test}{%
	\gdef\@journal{test}
	\gdef\@journalfull{TEST}
	\gdef\@journalshort{TEST}
	\gdef\@doiabbr{test}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
